Gautschi-type and implicit-explicit integrators for constrained wave equations

This paper deals with the construction and analysis of two integrators for (semi-linear) second-order partial differential-algebraic equations of semi-explicit type. More precisely, we consider an implicit-explicit Crank-Nicolson scheme as well as an exponential integrator of Gautschi type. For this, well-known wave integrators for unconstrained systems are combined with techniques known from the field of differential-algebraic equations. This results in efficient time stepping schemes that are provable of second order. Moreover, we discuss the practical implementation of the Gautschi-type method, which involves the solution of certain saddle point problems. The theoretical results are verified by a numerical experiment for the wave equation with kinetic boundary conditions.

==> plot_convDynBC_H1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=\columnwidth,
height=\columnwidth,
%at={(1.625in,0.573in)},
scale only axis,
xmode=log,
xmin=0.0002,
xmax=0.3,
xminorticks=true,
%xlabel style={font=\color{white!15!black}},
xlabel={time step size $\tau$},
ymode=log,
ymin=1.2e-08,
ymax=4,
yminorticks=true,
%ylabel={$\|u - u^n_h \|_{L^\infty(0,T;L^2(\Omega))}$}, 
ylabel={error in $u$}, % $L^\infty(0,T;L^2(\Omega))$ 
axis background/.style={fill=white},
title style={font=\bfseries},
%title={$\|u-(u^n)^\ell\|_{L^\infty(L^2)}$},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=mycolor1, line width=1.5pt, mark=*, mark size=2.5]
 table[row sep=crcr]{%
	0.5	0.886897811423382\\
	0.25	0.814001455719381\\
	0.125	0.71842292468621\\
	0.0625	0.59668495735049\\
	0.03125	0.462722249104853\\
	0.015625	0.335124218810381\\
	0.0078125	0.226355091442213\\
	0.00390625	0.142846882477949\\
	0.001953125	0.0854833231860771\\
	0.0009765625	0.0496951576200541\\
	0.00048828125	0.0285061358386572\\
	0.000244140625	0.0159631324361717\\
};
\addlegendentry{IMEX Euler} % lvl 6 (h=0.067169)

\addplot [color=mycolor2, line width=1.5pt, mark=triangle*, mark size=3.0]
table[row sep=crcr]{%
	0.5	1.1399231149206\\
	0.25	0.911185070890152\\
	0.125	0.600641640562755\\
	0.0625	0.34278508529489\\
	0.03125	0.150659820505709\\
	0.015625	0.0629253350632058\\
	0.0078125	0.0338056316346295\\
	0.00390625	0.0119280239891894\\
	0.001953125	0.00307543174055201\\
	0.0009765625	0.000770735400661403\\
	0.00048828125	0.000192738372290943\\
	0.000244140625	4.81875108325731e-05\\
};
\addlegendentry{IMEX CN} % lvl 6 (h=0.067169)

\addplot [color=mycolor3, line width=1.5pt, mark=square*, mark size=2.8]
table[row sep=crcr]{%
%	0.5	12.592173\\
	0.25	2.4557014\\
	0.125	1.3502588\\
	0.0625	0.48398435\\
	0.03125	0.23941442\\
	0.015625	0.0099419191\\
	0.0078125	0.0024957581\\
	0.00390625	0.00062673088\\
	0.001953125	0.00015693559\\
	0.0009765625	3.926216e-05\\
	0.00048828125	9.8198502e-06\\
	0.000244140625	2.4564866e-06\\
};
\addlegendentry{Gautschi ($r=5$)} % lvl 6 (h=0.067169), KrylovDim = 5

% new for revision: leap-frog

\addplot [color=mycolor5, line width=1.5pt, mark=diamond*, mark size=2.]
table[row sep=crcr]{%
0.015625	0.0418325451779833\\
0.0078125	0.0223633704212942\\
0.00390625	0.00608730970336999\\
0.001953125	0.0015343823059839\\
0.0009765625	0.000384482527505693\\
0.00048828125	9.62353280607844e-05\\
0.000244140625	2.40706606765982e-05\\
};
\addlegendentry{leap-frog} % lvl 6 (h=0.067169)

%%%%%%%%%%%%%%%%%%%  orders  %%%%%%%%%%%%%

\addplot [color=gray, dashed, line width=1.25pt, forget plot]
table[row sep=crcr]{%
%	0.5	0.5\\
	0.25	0.25\\
%	0.125	0.125\\
%	0.0625	0.0625\\
%	0.03125	0.03125\\
%	0.015625	0.015625\\
%	0.0078125	0.0078125\\
%	0.00390625	0.00390625\\
%	0.001953125	0.001953125\\
%	0.0009765625	0.0009765625\\
	0.00048828125	0.00048828125\\
	0.000244140625	0.000244140625\\
};

\addplot [color=gray, dotted, line width=1.25pt, forget plot]
  table[row sep=crcr]{%
%	0.5	0.25\\
	0.25	0.0625\\
%	0.125	0.015625\\
%	0.0625	0.00390625\\
%	0.03125	0.0009765625\\
%	0.015625	0.000244140625\\
%	0.0078125	6.103515625e-05\\
%	0.00390625	1.52587890625e-05\\
%	0.001953125	3.814697265625e-06\\
%	0.0009765625	9.5367431640625e-07\\
	0.00048828125	2.38418579101562e-07\\
	0.000244140625	5.8276953e-08\\
};

\end{axis}

\end{tikzpicture}%

